High-dimensional Optimization with Low Rank Tensor Sampling and Local Search

We present a novel method called TESALOCS (TEnsor SAmpling and LOCal Search) for multidimensional optimization, combining the strengths of gradient-free discrete methods and gradient-based approaches. The discrete optimization in our method is based on low-rank tensor techniques, which, thanks to their low-parameter representation, enable efficient optimization of high-dimensional problems. For the second part, i.e., local search, any effective gradient-based method can be used, whether existing (such as quasi-Newton methods) or any other developed in the future. Our approach addresses the limitations of gradient-based methods, such as getting stuck in local optima; the limitations of discrete methods, which cannot be directly applied to continuous functions; and limitations of gradient-free methods that require large computational budgets. Note that we are not limited to a single type of low-rank tensor decomposition for discrete optimization, but for illustrative purposes, we consider a specific efficient low-rank tensor train decomposition. For 20 challenging 100-dimensional functions, we demonstrate that our method can significantly outperform results obtained with gradient-based methods like Conjugate Gradient, BFGS, SLSQP, and other methods, improving them by orders of magnitude with the same computing budget.

==> helpers.tex <==
% -------
% Helpers
\makeatletter

% \fat - bold font inside the formula or text:
\newcommand{\fat}[1]{\ifmmode\bm{#1}\else\textbf{#1}\fi}

% \set - linear/functional space (R, N, ...):
\newcommand{\set}[1]{\mathbb{#1}}

% \vect - vector:
\newcommand{\vect}[1]{\ensuremath{\fat{#1}}}

% \matr - matrix:
\newcommand{\matr}[1]{#1}

% \tens - tensor (or TT-tensor):
\newcommand{\tens}[1]{\mathcal{#1}}

% \qvect - QTT-vector:
\newcommand{\qvect}[1]{\mathbcal{#1}}

% \qmatr - QTT-matrix:
\newcommand{\qmatr}[1]{\mathcal{#1}}

% \func - function:
\newcommand{\func}[1]{\textsf{#1}}

% \vfunc - vector-function:
\newcommand{\vfunc}[1]{\textsf{\vect{#1}}}

% \ffunc - functional:
\newcommand{\ffunc}[1]{\widehat{#1}}

% \oper - operator:
\newcommand{\oper}[1]{\widehat{#1}}

% \trace - trace of the matrix:
\newcommand{\trace}[1]{\mathrm{Tr}\left( #1 \right)}

% \order - Operator O(...):
\newcommand{\order}[1]{\mathcal{O}\left( #1 \right)}

% \divergence - operator divergence(...):
\newcommand{\divergence}[1]{\mathrm{div}\left[ #1 \right]}

% \der - derivative d * / d *:
\newcommand{\der}[2]{\frac{d \, #1}{d \, #2}}

% \dert - time derivative d * / d t:
\newcommand{\dert}[1]{\der{#1}{t}}

% \derx - spatial derivative d * / d x:
\newcommand{\derx}[1]{\der{#1}{x}}

% \pder - partial derivative d * / d *:
\newcommand{\pder}[2]{\frac{\partial #1}{\partial #2}}

% \pdert - partial time derivative d * / d t:
\newcommand{\pdert}[1]{\pder{#1}{t}}

% \pderx - partial spatial derivative d * / d x:
\newcommand{\pderx}[1]{\pder{#1}{x}}

% \pderxi - partial spatial derivative for i-th component:
\newcommand{\pderxi}[2]{\pder{#1}{\vect{x}_{#2}}}

% \vectorize - vectorization (tensor to vector):
\newcommand{\vectorize}[1]{\fat{vec}\left( #1 \right)}

% \vectl - vector, represented as a list of its elements:
\newcommand{\vectl}[1]{\fat{\left[} #1 \fat{\right]}^{\top}}

% \iflatten - flatten index from multi-index:
\newcommand{\iflatten}[1]{\mathrm{ind}\left( #1 \right)}

% \imulti - multi-index from the flatten index:
\newcommand{\imulti}[1]{\fat{mind}\left( #1 \right)}

% \poi : point (dot) placeholder:
\newcommand{\poi}[0]{\, \cdot \,}

% \note - note (for review):
\newcommand{\note}[1]{ {\color[HTML]{8b1d1d}/* #1 */} }


% ---------
% Shortcuts

\newcommand{\vg}[0]{\vect{g}}            % Vector g
\newcommand{\vi}[0]{\vect{i}}            % Vector i
\newcommand{\vw}[0]{\vect{w}}            % Vector w
\newcommand{\vx}[0]{\vect{x}}            % Vector x
\newcommand{\vy}[0]{\vect{y}}            % Vector y
\newcommand{\vz}[0]{\vect{z}}            % Vector z

\newcommand{\mg}[0]{\matr{G}}            % Matrix g
\newcommand{\mw}[0]{\matr{W}}            % Matrix w
\newcommand{\mx}[0]{\matr{X}}            % Matrix x
\newcommand{\my}[0]{\matr{Y}}            % Matrix y
\newcommand{\mz}[0]{\matr{Z}}            % Matrix z

\newcommand{\tg}[0]{\tens{G}}            % Tensor G
\newcommand{\tw}[0]{\tens{W}}            % Tensor w
\newcommand{\tx}[0]{\tens{X}}            % Tensor x
\newcommand{\ty}[0]{\tens{Y}}            % Tensor y
\newcommand{\tz}[0]{\tens{Z}}            % Tensor z
\newcommand{\tp}[0]{\tens{P}}            % Tensor P

\newcommand{\tT}[0]{\tens{T}}            % Tensor P

\newcommand{\ff}[0]{\func{f}}            % Function f
\newcommand{\hff}[0]{\widehat{\ff}}      % Function hat f

\let\div=\relax
\DeclareMathOperator{\div}{div}
\DeclareMathOperator{\vecop}{vec}


% -------
% Various

% \newcommand{\fix}{\marginpar{FIX}}
% \newcommand{\new}{\marginpar{NEW}}
